Temporal Logic Specification-Conditioned Decision Transformer for Offline Safe Reinforcement Learning

Offline safe reinforcement learning (RL) aims to train a constraint satisfaction policy from a fixed dataset. Current state-of-the-art approaches are based on supervised learning with a conditioned policy. However, these approaches fall short in real-world applications that involve complex tasks with rich temporal and logical structures. In this paper, we propose temporal logic Specification-conditioned Decision Transformer (SDT), a novel framework that harnesses the expressive power of signal temporal logic (STL) to specify complex temporal rules that an agent should follow and the sequential modeling capability of Decision Transformer (DT). Empirical evaluations on the DSRL benchmarks demonstrate the better capacity of SDT in learning safe and high-reward policies compared with existing approaches. In addition, SDT shows good alignment with respect to different desired degrees of satisfaction of the STL specification that it is conditioned on.

==> tex_files/s5_theoretical-analysis.tex <==
\section{Theoretical Analysis}

In this section, we investigate the reason why decision transformers can be used to make decisions conditioned on the robustness values. 
We study this topic from two perspectives.
One is from the perspective of the expressivity of transformer networks while the other one is from the perspective of the Bayesian inference.

\subsection{Sufficient Expressivity for STL}
% \textbf{Sparsity in STL.}
% In many practical scenarios, a trajectory's compliance or violation of STL specifications might be determined by a relatively small number of critical states or intervals within the trajectory, which results in sparsity rewards ~\cite{bakhirkin2018efficient, meng2023signal}.
% For example, in a long signal sequence, only certain key segments might be critical for satisfying (or violating) the temporal logic criteria set by STL.
% % Sparse identification involves pinpointing these critical segments that have the most significant impact on the robustness value.
% This can be crucial for system diagnosis, understanding which parts of a signal are most responsible for specification compliance or failure, and for targeted signal processing or control strategy adjustments.

% \td{
% \begin{itemize}
%     \item Define some metrics to measure the sparsity, such as the percentage of key signal segments and how to identify key signal segments.
%     \item Why prefix and suffix? Intuitively, it makes sense, but it needs more rigorous analysis.
% \end{itemize}}



\subsection{STL as Prior Condition}
